H2LooP Telecom Model v1: From Telecom Comprehension to Autonomous Issue and PR Resolution

We present H2LooP Telecom Model v1, a domain-specialized large language models fine-tuned for the telecommunications industry. We release two domain-adapted model variants serving complementary use cases: a comprehension-focused variant for telecom domain question answering and reasoning, and an agentic variant for autonomous telecom code generation, pull request resolution, and code commits on production repositories. H2LooP Telecom achieves strong results on the GSMA Open Telecom Lite (OT-Lite) benchmark and a proprietary telecom code generation benchmark, outperforming frontier closed-source models such as GPT-5 and Claude Opus on independent leaderboard evaluation, while preserving general-purpose capabilities. The Comprehension variant achieves 81.8% weighted average on OT-Lite Pass@3, and, independently, ranks 5th overall on the official community-run Open Telco AI Leaderboard* at only 31B parameters-ahead of frontier closed-source systems including Claude Opus 4.6, GPT-5, Gemini 3 Flash, Grok-4-fast, and Kimi K2.5. Our agentic variant obtains a relative improvement of +8.8% in AST Similarity and +20.0% in Location IoU over the base model on telecom code generation, while maintaining identical MMLU (74.0%) and BFCL v3 multi-turn function calling (79.0%) performance, indicating zero catastrophic forgetting. Domain specialization on curated telecom corpora, spanning 3GPP standards, O-RAN specifications, network telemetry, and real repository commits, yields substantial improvements over general-purpose models of equivalent scale, approaches frontier closed-source models on domain-specific evaluation, and is independently corroborated by our official leaderboard standing.

==> sections/autonomous_pr.tex <==
\section{Autonomous PR Resolution}
\label{sec:autonomous_pr}

H2LooP Telecom Agent is designed for end-to-end autonomous pull request generation on telecom codebases. Given a natural language description of a required change (bug fix, feature addition, or standards-compliance update), the model executes the following pipeline:

\begin{enumerate}
    \item \textbf{File Localization:} Identifies relevant source files and code regions within the repository using learned structural priors about telecom project organization.
    \item \textbf{Edit Generation:} Produces syntactically correct, contextually appropriate code modifications conforming to project conventions and standards requirements.
    \item \textbf{Commit Structuring:} Organizes changes into coherent atomic commits with descriptive messages appropriate for code review.
\end{enumerate}

\subsection{Target Repositories}

We validate autonomous PR resolution capability across 11 production telecom repositories spanning the full software stack:

\begin{table}[H]
\centering
\caption{Target Repository Coverage.}
\label{tab:repos}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llll}
\toprule
\textbf{Repository} & \textbf{Domain} & \textbf{Language} & \textbf{Description} \\
\midrule
srsRAN 4G~\cite{srsran4g} & RAN & C/C++ & 4G/LTE software radio suite \\
srsRAN Project~\cite{srsranproject} & RAN & C++ & 5G NR RAN implementation \\
Open5GS~\cite{open5gs} & Core & C & 5G core network (AMF, SMF, UPF, etc.) \\
free5GC~\cite{free5gc} & Core & Go & 5G core network implementation \\
OpenAirInterface5G~\cite{oai} & RAN/Core & C & 5G reference implementation \\
UERANSIM~\cite{ueransim} & Simulation & C++ & 5G UE and gNB simulator \\
NVIDIA Aerial~\cite{aerial} & RAN & C++/CUDA & CUDA-accelerated L1/L2 \\
gr-gsm~\cite{grgsm} & Legacy & C++/Python & GNU Radio GSM receiver \\
LTE-Cell-Scanner~\cite{ltescanner,ltescanner2} & Tools & C++ & LTE cell search and synchronization \\
RIS-Codes-Collection~\cite{riscodes} & Research & MATLAB/Python & RIS algorithm implementations \\
\bottomrule
\end{tabular}%
}
\end{table}

The repository set covers five distinct programming languages (C, C++, Go, Python, MATLAB), four telecom stack layers (physical, RAN, core, simulation), and project sizes ranging from 50K to 2M+ lines of code. This diversity validates that the model's code generation capability generalizes across telecom software paradigms rather than overfitting to a single project structure or language.

\subsection{PR Resolution Pipeline}

The autonomous PR workflow integrates H2LooP Telecom Agent into a standard software development loop:

\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{images/fig15_pipeline.png}
    \caption{Autonomous PR resolution pipeline.}
    \label{fig:pipeline}
\end{figure}

Each pipeline stage corresponds to a measurable capability:

\begin{table}[H]
\centering
\caption{Pipeline Stage to Metric Mapping.}
\label{tab:pipeline_metrics}
\begin{tabular}{llc}
\toprule
\textbf{Pipeline Stage} & \textbf{Corresponding Metric} & \textbf{Score} \\
\midrule
Edit Planning (Localization) & Location IoU & 0.446 \\
Code Generation (Structural) & AST Similarity & 0.570 \\
Code Generation (Surface) & Edit-Distance Score & 0.519 \\
Overall Patch Quality & BLEU-4 & 0.338 \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Qualitative Analysis}

We observe the following qualitative properties of generated PRs across target repositories:

\begin{itemize}
    \item \textbf{Standards compliance:} Generated code correctly references 3GPP procedure definitions and implements protocol state transitions consistent with specification requirements.
    \item \textbf{Project convention adherence:} The model adapts to per-repository coding style including naming conventions, error handling patterns, and logging frameworks.
    \item \textbf{Multi-file coherence:} Changes spanning multiple files maintain consistency across header declarations, implementation bodies, and test modifications.
    \item \textbf{Build system awareness:} Generated edits account for build dependencies, CMake configurations, and conditional compilation directives.
\end{itemize}

